Beyond Fairness Metrics: Roadblocks and Challenges for Ethical AI in Practice

We review practical challenges in building and deploying ethical AI at the scale of contemporary industrial and societal uses. Apart from the purely technical concerns that are the usual focus of academic research, the operational challenges of inconsistent regulatory pressures, conflicting business goals, data quality issues, development processes, systems integration practices, and the scale of deployment all conspire to create new ethical risks. Such ethical concerns arising from these practical considerations are not adequately addressed by existing research results. We argue that a holistic consideration of ethics in the development and deployment of AI systems is necessary for building ethical AI in practice, and exhort researchers to consider the full operational contexts of AI systems when assessing ethical risks.

==> Makefile <==
MAIN=main
BIB=bib
OUTPUT_DIR=output
AUX_DIR=output_aux

.PHONY: all check link clean travis data tatoeba

pdf:
	latexmk -pdf $(MAIN) -auxdir=$(OUTPUT_DIR) -outdir=$(OUTPUT_DIR)

all: pdf
	make -C code/programs

check:
	chktex -n1 -n2 -n3 -n8 -n11 -n12 -n13 -n14 -n26 -n34 -n33 -n36 -n40 -n44 $(MAIN)
	biber --tool -V $(BIB).bib
	rm -f $(BIB)_bibertool.bib

lint:
	biber --tool $(BIB).bib --output-fieldcase=lower --isbn-normalise
	mv $(BIB)_bibertool.bib $(BIB).bib

arxiv: pdf
	mkdir -p arxiv
	cp *.pdf $(OUTPUT_DIR)/*.bbl *.bib *.tex *.cls *.bst arxiv
	#Download any new versions of packages here
	#e.g.
	#curl -L -o arxiv/algorithm2e.sty https://ctan.sharelatex.com/tex-archive/macros/latex/contrib/algorithm2e/tex/algorithm2e.sty
	#Test build
	cd arxiv && latexmk -pdf $(MAIN) -auxdir=arxivtest -outdir=arxivtest && rm -rf arxivtest
	cd arxiv && zip arxiv.zip *

clean:
	latexmk -c -pdf
	rm -rvf *.bbl *.blg *.aux *.fls *.fdb_latexmk *.log *.out *.toc $(MAIN).pdf $(AUX_DIR) $(OUTPUT_DIR) arxiv

travis:
	#Old latexmk doesn't understand auxdir and outdir options
	latexmk -pdf -pdflatex='pdflatex %S %O -interaction=nonstopmode -halt-on-error' $(MAIN)

######################
# Download data
######################
TATOEBA_CORPUS = data/tatoeba/users_sentences.csv \
	data/tatoeba/user_languages.csv \
data/tatoeba/sentences_in_lists.csv \
data/tatoeba/links.csv \
data/tatoeba/tags.csv \
data/tatoeba/sentences_detailed.csv \
data/tatoeba/user_lists.csv

data: $(TATOEBA_CORPUS)

tatoeba: $(TATOEBA_CORPUS)

data/tatoeba/users_sentences.csv:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/users_sentences.csv

data/tatoeba/%.csv: data/tatoeba/%.tar.bz2
	tar -xjvf $< -C data/tatoeba

data/tatoeba/%.tar.bz2:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/$(notdir $@)


